Benchmarking and Improving Text-to-SQL Generation under Ambiguity

Research in Text-to-SQL conversion has been largely benchmarked against datasets where each text query corresponds to one correct SQL. However, natural language queries over real-life databases frequently involve significant ambiguity about the intended SQL due to overlapping schema names and multiple confusing relationship paths. To bridge this gap, we develop a novel benchmark called AmbiQT with over 3000 examples where each text is interpretable as two plausible SQLs due to lexical and/or structural ambiguity. When faced with ambiguity, an ideal top-$k$ decoder should generate all valid interpretations for possible disambiguation by the user. We evaluate several Text-to-SQL systems and decoding algorithms, including those employing state-of-the-art LLMs, and find them to be far from this ideal. The primary reason is that the prevalent beam search algorithm and its variants, treat SQL queries as a string and produce unhelpful token-level diversity in the top-$k$. We propose LogicalBeam, a new decoding algorithm that navigates the SQL logic space using a blend of plan-based template generation and constrained infilling. Counterfactually generated plans diversify templates while in-filling with a beam-search that branches solely on schema names provides value diversity. LogicalBeam is up to $2.5$ times more effective than state-of-the-art models at generating all candidate SQLs in the top-$k$ ranked outputs. It also enhances the top-$5$ Exact and Execution Match Accuracies on SPIDER and Kaggle DBQA.

==> plot.tex <==
\begin{figure*}
\centering
\begin{tikzpicture}
\begin{groupplot}[group style={group size= 4 by 3,ylabels at=edge left},width=0.25\textwidth,height=0.18\textwidth]
\nextgroupplot[label style={font=\Large},
tick label style={font=\Large},
legend style={at={($(0,0)+(1cm,1cm)$)},legend columns=6,fill=none,draw=black,anchor=center,align=center},
ylabel = {AirQ},
legend to name=fred,
title = MCAR,
mark size=2pt]
\addplot[red!70!black,mark=*] coordinates {(10, 0.206) (40, 0.153) (70, 0.433) (100, 0.465) };
\addplot[brown,mark=star] coordinates {(10, 0.219) (40, 0.160) (70, 0.337) (100, 0.356) };
\addplot[cyan,mark=square*] coordinates {(10, 0.199) (40, 0.154) (70, 0.547) (100, 0.374) };
\addplot[gray,mark=triangle*] coordinates {(10, 0.197) (40, 0.155) (70, 0.384) (100, 0.463) };
\addplot[blue,mark=diamond*] coordinates {(10, 0.022) (40, 0.059) (70, 0.231) (100, 0.234) };
\addlegendentry{CDRec};    
\addlegendentry{DynaMMO};    
\addlegendentry{TRMF};          
\addlegendentry{SVDImp};          
\addlegendentry{\sysname};          
\coordinate (c1) at (rel axis cs:0,1);

\nextgroupplot[label style={font=\Large},
tick label style={font=\Large},
title = MissDisj,
mark size=2pt]
\addplot [red!70!black,mark=*] coordinates {(10, 0.061) (40, 0.214) (70, 0.436) (100, 0.531) };
\addplot [brown,mark=star] coordinates {(10, 0.063) (40, 0.232) (70, 0.356) (100, 0.416) };
\addplot [cyan,mark=square*] coordinates {(10, 0.054) (40, 0.231) (70, 0.573) (100, 0.492) };
\addplot [gray,mark=triangle*] coordinates {(10, 0.052) (40, 0.231) (70, 0.400) (100, 0.587) };
\addplot [blue,mark=diamond*] coordinates {(10, 0.070) (40, 0.062) (70, 0.228) (100, 0.302) };

\nextgroupplot[label style={font=\Large},
tick label style={font=\Large},
title = MissOver,
mark size=2pt]
\addplot [red!70!black,mark=*] coordinates {(10, 0.198) (40, 0.212) (70, 0.600) (100, 0.694) };
\addplot [brown,mark=star] coordinates {(10, 0.206) (40, 0.233) (70, 0.391) (100, 0.408) };
\addplot [cyan,mark=square*] coordinates {(10, 0.196) (40, 0.224) (70, 0.470) (100, 0.525) };
\addplot [gray,mark=triangle*] coordinates {(10, 0.188) (40, 0.224) (70, 0.556) (100, 0.645) };
\addplot [blue,mark=diamond*] coordinates {(10, 0.075) (40, 0.085) (70, 0.276) (100, 0.309) };

\nextgroupplot[label style={font=\Large},
tick label style={font=\Large},
title = Blackout,
ymax=1,
mark size=2pt]
\addplot [red!70!black,mark=*] coordinates {(10, 0.088) (40, 0.503) (70, 0.472) (100, 0.877) };
\addplot [brown,mark=star] coordinates {(10, 0.104) (40, 0.482) (70, 0.561) (100, 0.821) };
\addplot [cyan,mark=square*] coordinates {(10, 2.847) (40, 2.515) (70, 2.186) (100, 1.968) };
\addplot [gray,mark=triangle*] coordinates {(10, 0.715) (40, 0.660) (70, 0.719) (100, 0.883) };
\addplot [blue,mark=diamond*] coordinates {(10, 0.092) (40, 0.670) (70, 0.720) (100, 0.654) };

\coordinate (c2) at (rel axis cs:1,1);
\nextgroupplot[label style={font=\Large},
ylabel = {Climate},
tick label style={font=\Large},
mark size=2pt]
\addplot [red!70!black,mark=*] coordinates {(10, 0.699) (40, 0.707) (70, 0.607) (100, 0.591) };
\addplot [brown,mark=star] coordinates {(10, 0.571) (40, 0.592) (70, 0.535) (100, 0.542) };
\addplot [cyan,mark=square*] coordinates {(10, 0.674) (40, 0.693) (70, 0.593) (100, 0.589) };
\addplot [gray,mark=triangle*] coordinates {(10, 0.679) (40, 0.695) (70, 0.596) (100, 0.591) };
\addplot [blue,mark=diamond*] coordinates {(10, 0.167) (40, 0.234) (70, 0.244) (100, 0.275) };
% \addplot [blue,mark=diamond*] coordinates {(10, 0.167) (40, 0.284) (70, 0.298) (100, 0.340) };
\nextgroupplot[label style={font=\Large},
tick label style={font=\Large},
mark size=2pt]
\addplot [red!70!black,mark=*] coordinates {(10, 0.705) (40, 0.630) (70, 0.591) (100, 0.602) };
\addplot [brown,mark=star] coordinates {(10, 0.586) (40, 0.563) (70, 0.554) (100, 0.572) };
\addplot [cyan,mark=square*] coordinates {(10, 0.680) (40, 0.619) (70, 0.583) (100, 0.595) };
\addplot [gray,mark=triangle*] coordinates {(10, 0.685) (40, 0.620) (70, 0.584) (100, 0.597) };
\addplot [blue,mark=diamond*] coordinates {(10, 0.507) (40, 0.453) (70, 0.499) (100, 0.621) };
%\addplot coordinates {(10, 0.494) (40, 0.558) (70, 0.585) (100, 0.616) };

\nextgroupplot[label style={font=\Large},
tick label style={font=\Large},
mark size=2pt]
\addplot [red!70!black,mark=*] coordinates {(10, 0.720) (40, 0.765) (70, 0.678) (100, 0.666) };
\addplot [brown,mark=star] coordinates {(10, 0.622) (40, 0.667) (70, 0.610) (100, 0.613) };
\addplot [cyan,mark=square*] coordinates {(10, 0.689) (40, 0.758) (70, 0.659) (100, 0.649) };
\addplot [gray,mark=triangle*] coordinates {(10, 0.695) (40, 0.762) (70, 0.662) (100, 0.652) };
\addplot [blue,mark=diamond*] coordinates {(10, 0.466) (40, 0.706) (70, 0.679) (100, 0.677) };
%\addplot coordinates {(10, 0.495) (40, 0.701) (70, 0.675) (100, 0.677) };

\nextgroupplot[label style={font=\Large},
tick label style={font=\Large},
ymax=1,
mark size=2pt]
\addplot [red!70!black,mark=*] coordinates {(10, 0.714) (40, 0.629) (70, 0.797) (100, 0.728) };
\addplot [brown,mark=star] coordinates {(10, 0.564) (40, 0.700) (70, 0.798) (100, 0.781) };
\addplot [cyan,mark=square*] coordinates {(10, 2.941) (40, 3.144) (70, 3.181) (100, 3.284) };
\addplot [gray,mark=triangle*] coordinates {(10, 0.748) (40, 0.847) (70, 0.869) (100, 0.858) };
\addplot [blue,mark=diamond*] coordinates {(10, 0.269) (40, 0.303) (70, 0.383) (100, 0.379) };

\nextgroupplot[label style={font=\Large},
ylabel = {Electricity},
tick label style={font=\Large},
mark size=2pt,
xlabel = \% TS Incomplete]
\addplot [red!70!black,mark=*] coordinates {(10, 0.547) (40, 0.531) (70, 0.481) (100, 0.423) };
\addplot [brown,mark=star] coordinates {(10, 0.520) (40, 0.501) (70, 0.463) (100, 0.420) };
\addplot [cyan,mark=square*] coordinates {(10, 0.548) (40, 0.538) (70, 0.489) (100, 0.439) };
\addplot [gray,mark=triangle*] coordinates {(10, 0.549) (40, 0.540) (70, 0.491) (100, 0.440) };
\addplot [blue,mark=diamond*] coordinates {(10, 0.390) (40, 0.349) (70, 0.338) (100, 0.309) };
\nextgroupplot[label style={font=\Large},
tick label style={font=\Large},
mark size=2pt,
xlabel = \% TS Incomplete]
\addplot [red!70!black,mark=*] coordinates {(10, 0.549) (40, 0.592) (70, 0.493) (100, 0.442) };
\addplot [brown,mark=star] coordinates {(10, 0.472) (40, 0.557) (70, 0.466) (100, 0.423) };
\addplot [cyan,mark=square*] coordinates {(10, 0.527) (40, 0.593) (70, 0.489) (100, 0.440) };
\addplot [gray,mark=triangle*] coordinates {(10, 0.531) (40, 0.595) (70, 0.490) (100, 0.441) };
%\addplot coordinates {(10, 0.590) (40, 0.615) (70, 0.485) (100, 0.428) };
\addplot [blue,mark=diamond*] coordinates {(10, 0.482) (40, 0.535) (70, 0.394) (100, 0.377) };

\nextgroupplot[label style={font=\Large},
tick label style={font=\Large},
ymax=1,
mark size=2pt,
xlabel = \% TS Incomplete]
\addplot [red!70!black,mark=*] coordinates {(10, 0.565) (40, 0.613) (70, 0.508) (100, 0.459) };
\addplot [brown,mark=star] coordinates {(10, 0.457) (40, 0.602) (70, 0.503) (100, 0.458) };
\addplot [cyan,mark=square*] coordinates {(10, 0.539) (40, 1.284) (70, 0.895) (100, 0.737) };
\addplot [gray,mark=triangle*] coordinates {(10, 0.544) (40, 0.614) (70, 0.512) (100, 0.464) };
%\addplot coordinates {(10, 0.606) (40, 0.639) (70, 0.514) (100, 0.455) };
\addplot [blue,mark=diamond*] coordinates {(10, 0.617) (40, 0.589) (70, 0.523) (100, 0.457) };

\nextgroupplot[label style={font=\Large},
tick label style={font=\Large},
ymax=1,
mark size=2pt,
xlabel = Block Size]
\addplot [red!70!black,mark=*] coordinates {(10, 0.976) (40, 1.055) (70, 0.997) (100, 0.968) };
\addplot [brown,mark=star] coordinates {(10, 0.810) (40, 0.948) (70, 0.935) (100, 0.956) };
\addplot [cyan,mark=square*] coordinates {(10, 1.978) (40, 2.146) (70, 2.221) (100, 2.264) };
\addplot [gray,mark=triangle*] coordinates {(10, 1.208) (40, 1.124) (70, 1.051) (100, 1.058) };
\addplot [blue,mark=diamond*] coordinates {(10, 0.413) (40, 0.508) (70, 0.526) (100, 0.597) };


\end{groupplot}
\coordinate (c3) at ($(c1)!.5!(c2)$);
\node[below] at (c3 |- current bounding box.south)
%\path (c1-|current bounding box.west)-- node[anchor=south,rotate=90] {\Large Mean Absolute Error} (c4-|current bounding box.west);
{\pgfplotslegendfromname{fred}};

\end{tikzpicture}
\caption{Mean Absolute Errors (y-axis) on three datasets along  rows and under four missing scenarios along columns. X-axis is percent of time-series with a missing block for MCAR, MissDisj, MissOver and size of the missing block for Blackout.}
\label{fig:graph}
\end{figure*}
%\todo[inline]{Put captions similar to Fig 2 clearly describing axis and plots in all figures}

%\coordinate (c4) at (rel axis cs:0,0);

